Pathfinding Neural Cellular Automata

Pathfinding makes up an important sub-component of a broad range of complex tasks in AI, such as robot path planning, transport routing, and game playing. While classical algorithms can efficiently compute shortest paths, neural networks could be better suited to adapting these sub-routines to more complex and intractable tasks. As a step toward developing such networks, we hand-code and learn models for Breadth-First Search (BFS), i.e. shortest path finding, using the unified architectural framework of Neural Cellular Automata, which are iterative neural networks with equal-size inputs and outputs. Similarly, we present a neural implementation of Depth-First Search (DFS), and outline how it can be combined with neural BFS to produce an NCA for computing diameter of a graph. We experiment with architectural modifications inspired by these hand-coded NCAs, training networks from scratch to solve the diameter problem on grid mazes while exhibiting strong generalization ability. Finally, we introduce a scheme in which data points are mutated adversarially during training. We find that adversarially evolving mazes leads to increased generalization on out-of-distribution examples, while at the same time generating data-sets with significantly more complex solutions for reasoning tasks.

==> Tables/diameter_evo_data_cross_eval_selective.tex <==
\begin{tabular}{|c|r|r|r|r|r|r|r|r|}
\hline
    &       &     &     model & \multicolumn{2}{c|}{train} & \multicolumn{3}{c|}{test} \\
\cline{4-9}
\cline{4-9}
    &       &     &       --- & \multicolumn{2}{c|}{16x16} & \multicolumn{2}{c|}{16x16} &                   32x32 \\
\cline{4-9}
\cline{4-9}
    &       &     & n. params &                sol len &           pct. complete &             accuracies &          pct. complete &              accuracies \\
\textbf{model} & \textbf{env generation} & \textbf{n. hid chan} &           &                        &                         &                        &                        &                         \\
\hline
\multirow{4}{*}{\textbf{NCA}} & \multirow{2}{*}{\textbf{False}} & \textbf{96 } &    84,672 &           24.09 ± 0.00 &           71.58 ± 40.13 &          66.15 ± 36.99 &          55.66 ± 31.15 &           -5.20 ± 41.28 \\
    &       & \textbf{128} &   149,760 &           24.09 ± 0.00 &  \textbf{74.04} ± 41.39 &          67.20 ± 37.57 &          58.32 ± 32.60 &           27.47 ± 52.59 \\
\cline{2-9}
    & \multirow{2}{*}{\textbf{True }} & \textbf{96 } &    84,672 &           26.06 ± 1.11 &           33.94 ± 19.12 &          70.47 ± 39.40 &          52.90 ± 29.61 &  \textbf{60.01} ± 33.55 \\
    &       & \textbf{128} &   149,760 &  \textbf{27.43} ± 0.15 &            49.85 ± 4.07 &  \textbf{90.02} ± 0.44 &  \textbf{75.79} ± 1.57 &           30.02 ± 64.80 \\
\hline
\end{tabular}

==> Tables/diameter_kernel_cross_eval_selective.tex <==
% \begin{tabular}{|c|r|r|r|r|r|r|r|r|}
% \hline
%     &   &      &    &     model &                  train & \multicolumn{3}{c|}{test} \\
% \cline{5-9}
% \cline{5-9}
%     &   &      &    &       --- &                  16x16 &                  16x16 & \multicolumn{2}{c|}{32x32} \\
% \cline{5-9}
% \cline{5-9}
%     &   &      &    & n. params &          pct. complete &          pct. complete &                   accuracy &          pct. complete \\
% \textbf{model} & \textbf{kernel size} & \textbf{max pool} & \textbf{n. hid chan} &           &                        &                        &                        &                        \\
% \hline
% \multirow{8}{*}{\textbf{NCA}} & \multirow{4}{*}{\textbf{3}} & \multirow{2}{*}{\textbf{False}} & \textbf{48} &    21,600 &           50.28 ± 5.68 &           43.54 ± 5.31 &            9.68 ± 7.11 &            1.44 ± 1.46 \\
%     &   &      & \textbf{96} &    84,672 &  \textbf{90.93} ± 3.77 &           64.39 ± 6.38 &           25.65 ± 8.14 &           15.73 ± 4.01 \\
% \cline{3-9}
%     &   & \multirow{2}{*}{\textbf{True}} & \textbf{48} &    21,600 &           40.23 ± 5.64 &           35.03 ± 5.92 &          -18.73 ± 7.24 &            0.13 ± 0.48 \\
%     &   &      & \textbf{96} &    84,672 &           82.96 ± 4.56 &  \textbf{66.55} ± 6.14 &  \textbf{69.80} ± 5.71 &  \textbf{48.05} ± 6.32 \\
% \cline{2-9}
% \cline{3-9}
%     & \multirow{4}{*}{\textbf{5}} & \multirow{2}{*}{\textbf{False}} & \textbf{48} &    60,000 &           72.78 ± 5.99 &           51.32 ± 6.25 &            3.89 ± 5.86 &            2.76 ± 1.87 \\
%     &   &      & \textbf{96} &   235,200 &           85.57 ± 4.67 &           57.70 ± 5.72 &            9.37 ± 7.59 &            5.75 ± 3.03 \\
% \cline{3-9}
%     &   & \multirow{2}{*}{\textbf{True}} & \textbf{48} &    60,000 &           70.86 ± 5.87 &           49.21 ± 6.63 &            8.17 ± 7.48 &            5.22 ± 2.60 \\
%     &   &      & \textbf{96} &   235,200 &           89.04 ± 3.81 &           61.50 ± 5.96 &           -5.90 ± 7.89 &            1.89 ± 1.64 \\
% \hline
% \end{tabular}

\begin{tabular}{|c|r|r|r|r|r|r|r|r|}
\hline
    &   &     &       &     model &                  train & \multicolumn{3}{c|}{test} \\
\cline{5-9}
\cline{5-9}
    &   &     &       &       --- &                  16x16 &                  16x16 & \multicolumn{2}{c|}{32x32} \\
\cline{5-9}
\cline{5-9}
    &   &     &       & n. params &          pct. complete &          pct. complete &              accuracies &           pct. complete \\
\textbf{model} & \textbf{kernel size} & \textbf{n. hid chan} & \textbf{cut corners} &           &                        &                        &                         &                         \\
\hline
\multirow{4}{*}{\textbf{NCA}} & \multirow{2}{*}{\textbf{3}} & \multirow{2}{*}{\textbf{128}} & \textbf{False} &   149,760 &           56.56 ± 1.31 &           65.00 ± 6.59 &  \textbf{33.01} ± 16.62 &  \textbf{20.94} ± 12.23 \\
    &   &     & \textbf{True } &    83,200 &          43.12 ± 24.27 &          42.19 ± 24.08 &           27.99 ± 16.50 &             8.12 ± 8.44 \\
\cline{2-9}
\cline{3-9}
    & \multirow{2}{*}{\textbf{5}} & \multirow{2}{*}{\textbf{128}} & \textbf{False} &   416,000 &           58.75 ± 6.11 &           61.88 ± 6.11 &             7.19 ± 9.20 &             7.50 ± 2.80 \\
    &   &     & \textbf{True } &   216,320 &  \textbf{66.88} ± 6.39 &  \textbf{71.25} ± 4.22 &            19.97 ± 9.06 &            10.62 ± 6.29 \\
\hline
\end{tabular}

==> Tables/diameter_kernel_cross_eval_selective_0.tex <==
\begin{tabular}{|c|r|r|r|r|r|r|r|r|}
\hline
    &   &      &     &     model &                  train & \multicolumn{3}{c|}{test} \\
\cline{5-9}
\cline{5-9}
    &   &      &     &       --- &                  16x16 &                  16x16 & \multicolumn{2}{c|}{32x32} \\
\cline{5-9}
\cline{5-9}
    &   &      &     & n. params &          pct. complete &          pct. complete &             accuracies &          pct. complete \\
\textbf{model} & \textbf{kernel size} & \textbf{cut corners} & \textbf{n. hid chan} &           &                        &                        &                        &                        \\
\hline
\multirow{8}{*}{\textbf{NCA}} & \multirow{4}{*}{\textbf{3}} & \multirow{2}{*}{\textbf{False}} & \textbf{96 } &    84,672 &           80.77 ± 5.51 &           67.00 ± 5.55 &          -28.80 ± 7.81 &            0.11 ± 0.44 \\
    &   &      & \textbf{128} &   149,760 &           79.08 ± 4.78 &           66.62 ± 6.20 &          -26.12 ± 8.82 &            0.10 ± 0.38 \\
\cline{3-9}
    &   & \multirow{2}{*}{\textbf{True}} & \textbf{96 } &    47,040 &           11.40 ± 3.70 &           11.18 ± 3.72 &           24.24 ± 6.39 &            1.40 ± 1.47 \\
    &   &      & \textbf{128} &    83,200 &           74.98 ± 5.29 &  \textbf{67.82} ± 5.99 &           -3.09 ± 6.98 &            1.64 ± 1.56 \\
\cline{2-9}
\cline{3-9}
    & \multirow{4}{*}{\textbf{5}} & \multirow{2}{*}{\textbf{False}} & \textbf{96 } &   235,200 &           87.55 ± 3.85 &           63.44 ± 6.08 &          -17.54 ± 7.35 &            0.54 ± 0.95 \\
    &   &      & \textbf{128} &   416,000 &  \textbf{88.84} ± 3.58 &           66.41 ± 5.94 &            8.34 ± 7.83 &            5.52 ± 2.76 \\
\cline{3-9}
    &   & \multirow{2}{*}{\textbf{True}} & \textbf{96 } &   122,304 &           83.85 ± 4.35 &           67.22 ± 5.29 &          -22.10 ± 7.81 &            0.34 ± 0.69 \\
    &   &      & \textbf{128} &   216,320 &           87.65 ± 4.37 &           67.47 ± 6.32 &  \textbf{54.13} ± 6.83 &  \textbf{35.63} ± 6.27 \\
\hline
\end{tabular}

==> Tables/loss_interval_cross_eval.tex <==
\begin{tabular}{|c|r|r|r|r|r|}
\hline
    &    & \multicolumn{2}{c|}{train} & \multicolumn{2}{c|}{test} \\
\cline{3-6}
    &    &          pct. complete &       completion time &          pct. complete &       completion time \\
\textbf{model} & \textbf{loss interval} &                        &                       &                        &                       \\
\hline
\multirow{5}{*}{\textbf{NCA}} & \textbf{4 } &           93.46 ± 2.80 &           6.51 ± 3.07 &           82.28 ± 4.62 &           6.94 ± 3.25 \\
    & \textbf{8 } &           99.02 ± 1.16 &           6.04 ± 3.06 &           90.33 ± 3.84 &           6.32 ± 3.20 \\
    & \textbf{16} &  \textbf{99.90} ± 0.54 &  \textbf{5.83} ± 3.24 &           93.99 ± 2.03 &  \textbf{5.87} ± 3.40 \\
    & \textbf{32} &           99.46 ± 0.84 &           6.29 ± 2.80 &  \textbf{94.19} ± 2.22 &           6.39 ± 2.89 \\
    & \textbf{64} &           95.85 ± 2.64 &           6.05 ± 3.20 &           86.87 ± 4.04 &           6.22 ± 3.38 \\
\hline
\end{tabular}

==> Tables/models_cross_eval_0.tex <==
\begin{tabular}{|c|r|r|r|r|r|r|}
\hline
    &    &      model & \multicolumn{2}{c|}{train} & \multicolumn{2}{c|}{test} \\
\cline{3-7}
    &    &  n. params &                   accs &          pct. complete &                   accs &          pct. complete \\
\textbf{model} & \textbf{n layers} &            &                        &                        &                        &                        \\
\hline
\multirow{5}{*}{\textbf{MLP}} & \textbf{4 } &  1,661,728 &           79.12 ± 1.82 &           46.97 ± 7.83 &            5.01 ± 1.66 &            0.44 ± 0.80 \\
    & \textbf{8 } &  1,661,728 &           84.72 ± 2.03 &           43.80 ± 6.59 &            1.80 ± 2.33 &            0.15 ± 0.46 \\
    & \textbf{16} &  1,661,728 &           86.42 ± 2.08 &           42.82 ± 5.65 &            3.45 ± 1.44 &            0.39 ± 0.87 \\
    & \textbf{32} &  1,661,728 &  \textbf{88.57} ± 1.63 &           49.27 ± 5.27 &            1.58 ± 2.32 &            0.29 ± 0.72 \\
    & \textbf{64} &  1,661,728 &           86.98 ± 1.60 &           43.80 ± 5.36 &            1.11 ± 2.40 &            0.24 ± 0.57 \\
\cline{1-7}
\multirow{5}{*}{\textbf{NCA}} & \textbf{4 } &        872 &           51.86 ± 2.91 &           22.75 ± 5.03 &           50.91 ± 3.00 &           21.63 ± 5.51 \\
    & \textbf{8 } &        872 &           56.80 ± 3.87 &           29.00 ± 4.38 &           56.12 ± 4.11 &           29.59 ± 4.65 \\
    & \textbf{16} &        872 &           67.68 ± 3.46 &           43.95 ± 5.27 &           64.62 ± 4.49 &           41.80 ± 6.11 \\
    & \textbf{32} &        872 &           76.23 ± 3.73 &  \textbf{57.13} ± 6.38 &  \textbf{72.49} ± 4.98 &  \textbf{54.59} ± 6.33 \\
    & \textbf{64} &        872 &           68.54 ± 4.71 &           47.95 ± 5.05 &           66.26 ± 4.63 &           46.14 ± 6.81 \\
\hline
\end{tabular}

==> Tables/pathfinding_max_pool_cross_eval_selective.tex <==
% \begin{tabular}{|c|r|r|r|r|r|r|r|}
% \hline
%     &      &    &     model &                  train & \multicolumn{3}{c|}{test} \\
% \cline{4-8}
% \cline{4-8}
%     &      &    &       --- &                  16x16 &                  16x16 & \multicolumn{2}{c|}{32x32} \\
% \cline{4-8}
% \cline{4-8}
%     &      &    & n. params &          pct. complete &          pct. complete &                   accuracy &          pct. complete \\
% \textbf{model} & \textbf{max pool} & \textbf{n. hid chan} &           &                        &                        &                        &                        \\
% \hline
% \multirow{4}{*}{\textbf{NCA}} & \multirow{2}{*}{\textbf{False}} & \textbf{48} &    22,464 &           98.43 ± 1.58 &           96.53 ± 2.37 &  \textbf{88.98} ± 5.41 &           90.08 ± 3.45 \\
%     &      & \textbf{96} &    86,496 &  \textbf{99.12} ± 1.17 &  \textbf{97.55} ± 2.02 &           87.37 ± 6.07 &           90.25 ± 3.46 \\
% \cline{2-8}
%     & \multirow{2}{*}{\textbf{True}} & \textbf{48} &    22,464 &           98.50 ± 1.60 &           96.22 ± 2.23 &           87.79 ± 6.44 &  \textbf{91.30} ± 3.63 \\
%     &      & \textbf{96} &    86,400 &           98.43 ± 1.44 &           96.58 ± 2.41 &           86.52 ± 6.33 &           89.33 ± 3.95 \\
% \hline
% \end{tabular}

\begin{tabular}{|c|r|r|r|r|r|r|r|}
\hline
    &       &     &     model &                  train & \multicolumn{3}{c|}{test} \\
\cline{4-8}
\cline{4-8}
    &       &     &       --- &                  16x16 &                  16x16 & \multicolumn{2}{c|}{32x32} \\
\cline{4-8}
\cline{4-8}
    &       &     & n. params &          pct. complete &          pct. complete &             accuracies &          pct. complete \\
\textbf{model} & \textbf{max pool} & \textbf{n. hid chan} &           &                        &                        &                        &                        \\
\hline
\multirow{4}{*}{\textbf{NCA}} & \multirow{2}{*}{\textbf{False}} & \textbf{96 } &    86,400 &          78.53 ± 43.92 &          76.85 ± 42.97 &          66.05 ± 37.73 &          68.10 ± 38.22 \\
    &       & \textbf{128} &   152,064 &  \textbf{99.36} ± 0.24 &           97.61 ± 0.20 &  \textbf{90.06} ± 2.93 &           90.34 ± 1.64 \\
\cline{2-8}
    & \multirow{2}{*}{\textbf{True }} & \textbf{96 } &    86,400 &           98.22 ± 1.10 &           96.46 ± 0.94 &           83.49 ± 2.66 &           88.18 ± 2.13 \\
    &       & \textbf{128} &   152,064 &           99.22 ± 0.46 &  \textbf{97.64} ± 0.42 &           88.39 ± 3.15 &  \textbf{92.13} ± 1.19 \\
\hline
\end{tabular}

==> Tables/pathfinding_models_cross_eval_selective.tex <==
\begin{tabular}{|c|r|r|r|r|r|r|r|}
\hline
    &    &     &       model &                   train & \multicolumn{3}{c|}{test} \\
\cline{4-8}
\cline{4-8}
    &    &     &         --- &                   16x16 & \multicolumn{2}{c|}{16x16} &                  32x32 \\
\cline{4-8}
\cline{4-8}
    &    &     &   n. params &           pct. complete &                   accuracy &          pct. complete &          pct. complete \\
\textbf{model} & \textbf{n layers} & \textbf{n. hid chan} &             &                         &                        &                        &                        \\
\hline
\multirow{2}{*}{\textbf{GCN}} & \multirow{2}{*}{\textbf{16}} & \textbf{96 } &       9,600 &            13.12 ± 3.75 &           31.15 ± 2.17 &           13.33 ± 4.20 &            0.12 ± 0.42 \\
    &    & \textbf{256} &      66,560 &            19.80 ± 3.95 &           37.22 ± 2.44 &           19.67 ± 4.40 &            0.45 ± 0.85 \\
\cline{1-8}
\cline{2-8}
\multirow{2}{*}{\textbf{MLP}} & \multirow{2}{*}{\textbf{16}} & \textbf{96 } &  16,257,024 &            31.60 ± 6.36 &           15.03 ± 2.96 &            2.78 ± 2.12 &                    --- \\
    &    & \textbf{256} &  42,799,104 &            20.53 ± 5.41 &            6.86 ± 3.02 &            1.97 ± 1.90 &                    --- \\
\cline{1-8}
\cline{2-8}
\multirow{2}{*}{\textbf{NCA}} & \multirow{2}{*}{\textbf{16}} & \textbf{96 } &      86,400 &            99.76 ± 0.63 &           94.99 ± 2.74 &           92.98 ± 2.98 &           86.23 ± 4.26 \\
    &    & \textbf{256} &     599,040 &  \textbf{100.00} ± 0.00 &  \textbf{97.18} ± 2.12 &  \textbf{96.53} ± 2.15 &  \textbf{90.47} ± 3.67 \\
\hline
\end{tabular}

==> modif.tex <==
What to do next?
\begin{itemize}
\item Have a comparison with NCA including all the modifications and NCA not including any
\begin{itemize}
\item Put into contributions part of the introduction and Sec.2
\end{itemize}
\item Small (few hidden channels) weight sharing, and cut corner results for a graph of pct complete vs number of parameters (x-axis <- pct_complete)
\begin{itemize}
\item Combine the graphs and put the algorithm next to it
\end{itemize}
\item XXX Write a description for the diamater algorithm

\item  Put disccussion of the environment generalization, 16x16 follows the pattern but 32x32 not. Environment generalization does not help 32 x32  (data  do not hold huh)

\item XXX Graphs for weight sharing +cut corner might be wrong, maybe just two tables for that

\item Weight sharing diameter table 

\item XXX Change the table settings, focus on 16 x16 

\item Update big path finding
\end{itemize}


Order of diameter experiments (arch. mods):
\begin{itemize}
% \item Cutting corners of 3x3 kernels doesn't work (could exclude this result)
\item Max-pooling helps
\item Cutting corners helps
\item Kernel size does not help
\item With max-pooling on, (kernel size 3 or 5), cutting corners helps
\end{itemize}


What has been done?
